Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo

Riemannian manifold Hamiltonian Monte Carlo (RMHMC) is a powerful method of Bayesian inference that exploits underlying geometric information of the posterior distribution in order to efficiently traverse the parameter space. However, the form of the Hamiltonian necessitates complicated numerical integrators, such as the generalized leapfrog method, that preserve the detailed balance condition. The distinguishing feature of these numerical integrators is that they involve solutions to implicitly defined equations. Lagrangian Monte Carlo (LMC) proposes to eliminate the fixed point iterations by transitioning from the Hamiltonian formalism to Lagrangian dynamics, wherein a fully explicit integrator is available. This work makes several contributions regarding the numerical integrator used in LMC. First, it has been claimed in the literature that the integrator is only first-order accurate for the Lagrangian equations of motion; to the contrary, we show that the LMC integrator enjoys second order accuracy. Second, the current conception of LMC requires four determinant computations in every step in order to maintain detailed balance; we propose a simple modification to the integration procedure in LMC in order to reduce the number of determinant computations from four to two while still retaining a fully explicit numerical integration scheme. Third, we demonstrate that the LMC integrator enjoys a certain robustness to human error that is not shared with the generalized leapfrog integrator, which can invalidate detailed balance in the latter case. We discuss these contributions within the context of several benchmark Bayesian inference tasks.

==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/algorithms/generalized-leapfrog.tex <==
\begin{algorithm}[t!]
\caption{Pseudo-code implementing the generalized leapfrog integrator for computing approximate solutions to Hamilton's equations of motion. We assume a Hamiltonian in the form of \cref{lagrangian-remarks:eq:hamiltonian-form}.}
\label{lagrangian-remarks:alg:generalized-leapfrog}
\begin{algorithmic}[1]
  \STATE {\bf Input}: An integration step-size $\epsilon\in\R$, an initial position in phase space $(q, p)\in \R^m\times\R^m$.
  \STATE Compute an implicit half-step update to the momentum variable to obtain $\breve{p}$ using \cref{lagrangian-remarks:eq:generalized-leapfrog-momentum-i}.
  \STATE Compute an implicit full-step to the position variable to obtain $\tilde{q}$ using \cref{lagrangian-remarks:eq:generalized-leapfrog-position}.
  \STATE Compute an explicit half-step update to the momentum variable to obtain $\tilde{p}$ using \cref{lagrangian-remarks:eq:generalized-leapfrog-momentum-ii}.
  \STATE Compute the Jacobian determinant $J=1$.
  \STATE {\bf Output}: The updated position and momentum $(\tilde{q}, \tilde{p})$ and the Jacobian determinant $J$.
\end{algorithmic}
\end{algorithm}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/algorithms/hmc.tex <==
\begin{algorithm}[t!]
\caption{Single step of the Hamiltonian / Lagrangian Monte Carlo transition kernel.}
\label{lagrangian-remarks:alg:hmc}
\begin{algorithmic}[1]
  \STATE {\bf Input}: The current state of the Markov chain $(q_n, p_n)$, an integration step-size $\epsilon\in\R$, a number of integration steps $k\in\mathbb{N}$, a numerical integrator $\Phi$ (as described in any of \cref{lagrangian-remarks:alg:generalized-leapfrog,lagrangian-remarks:alg:lagrangian-leapfrog,lagrangian-remarks:alg:inverted-lagrangian-leapfrog}).
  \STATE Resample the momentum $p_n\vert q_n \sim \mathrm{Normal}(0, \mathbf{G}(q_n))$.
  \STATE Initialize the Jacobian determinant $J=1$ and initial integration state $(\tilde{q},\tilde{p}) = (q_n, p_n)$.
  \FOR{$i = 1,\ldots, k$}
  \STATE Compute the proposal by applying the numerical integrator: $((\tilde{q}, \tilde{p}), \tilde{J}) = \Phi_{\epsilon}(\tilde{q}, \tilde{p})$.
  \STATE Update the Jacobian determinant $J = J \times \tilde{J}$
  \ENDFOR
  \STATE Apply the momentum flip operator (\cref{lagrangian-remarks:def:momentum-flip}) to obtain $(\tilde{q}, \tilde{p}) = \mathbf{F}(\tilde{q}, \tilde{p})$.
  \STATE Sample $u\sim\mathrm{Uniform}(0, 1)$ and compute the acceptance probability $a = \alpha((q_n, p_n), (\tilde{q}, \tilde{p}), J)$ using \cref{lagrangian-remarks:eq:acceptance-probability}.
  \IF{$u < a$}
  \STATE Accept the proposal $(q_{n+1}, p_{n+1}) = (\tilde{q}, \tilde{p})$.
  \ELSE
  \STATE Reject the proposal $(q_{n+1}, p_{n+1}) = (q_n, p_n)$.
  \ENDIF
  \STATE {\bf Output}: The next state of the Markov chain $(q_{n+1}, p_{n+1})$.
\end{algorithmic}
\end{algorithm}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/algorithms/inverted-lagrangian-leapfrog.tex <==
\begin{algorithm}[t!]
\caption{Pseudo-code implementing the inverted Lagrangian leapfrog integrator for computing approximate solutions to the Lagrangian equations of motion. We assume a Lagrangian in the form of \cref{lagrangian-remarks:eq:lagrangian-form}. This version of leapfrog integration for Lagrangian dynamics requires only two Jacobian determinant computations in each step, as opposed to the four required by \cref{lagrangian-remarks:alg:lagrangian-leapfrog}.}
\label{lagrangian-remarks:alg:inverted-lagrangian-leapfrog}
\begin{algorithmic}[1]
  \STATE {\bf Input}: An integration step-size $\epsilon\in\R$, an initial position in phase space $(q, p)\in \R^m\times\R^m$.
  \STATE Use the inverse Legendre transform (\cref{lagrangian-remarks:def:inverse-legendre-transform}) to convert from momentum to velocity $v = \mathbf{G}^{-1}(q) p$.
  \STATE Compute an explicit half-step to the position variable to obtain $\breve{v}$ using \cref{lagrangian-remarks:eq:inverted-lagrangian-position-i}.
  \STATE Compute an explicit full-step update to the velocity variable to obtain $\tilde{v}$ using \cref{lagrangian-remarks:eq:inverted-lagrangian-velocity}.
  \STATE Compute an explicit half-step to the position variable to obtain $\tilde{q}$ using \cref{lagrangian-remarks:eq:inverted-lagrangian-position-ii}.
  \STATE Use the Legendre transform (\cref{lagrangian-remarks:def:legendre-transform}) to convert from velocity to momentum $\tilde{p} = \mathbf{G}(\tilde{q}) \tilde{v}$.
  \STATE Compute the Jacobian determinant $J = \frac{\partial (\tilde{q},\tilde{p})}{\partial (q, p)}$ using \cref{lagrangian-remarks:eq:lagrangian-jacobian-determinant}.
  \STATE {\bf Output}: The updated position and momentum $(\tilde{q}, \tilde{p})$ and the Jacobian determinant $J$.
\end{algorithmic}
\end{algorithm}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/algorithms/lagrangian-leapfrog.tex <==
\begin{algorithm}[t!]
\caption{Pseudo-code implementing the Lagrangian leapfrog integrator for computing approximate solutions to the Lagrangian equations of motion. We assume a Lagrangian in the form of \cref{lagrangian-remarks:eq:lagrangian-form}. The conversion from momentum to velocity and back again is included for notational simplicity; in practice, when applying multiple steps of this integrator, these conversions need only be computed for the first conversion from momentum to velocity and the last conversion from velocity to momentum.}
\label{lagrangian-remarks:alg:lagrangian-leapfrog}
\begin{algorithmic}[1]
  \STATE {\bf Input}: An integration step-size $\epsilon\in\R$, an initial position in phase space $(q, p)\in \R^m\times\R^m$.
  \STATE Use the inverse Legendre transform (\cref{lagrangian-remarks:def:inverse-legendre-transform}) to convert from momentum to velocity $v = \mathbf{G}^{-1}(q) p$.
  \STATE Compute an explicit half-step update to the velocity variable to obtain $\breve{v}$ using \cref{lagrangian-remarks:eq:lagrangian-velocity-i}.
  \STATE Compute an explicit full-step to the position variable to obtain $\tilde{q}$ using \cref{lagrangian-remarks:eq:lagrangian-position-update}.
  \STATE Compute an explicit half-step update to the velocity variable to obtain $\tilde{v}$ using \cref{lagrangian-remarks:eq:lagrangian-velocity-ii}.
  \STATE Use the Legendre transform (\cref{lagrangian-remarks:def:legendre-transform}) to convert from velocity to momentum $\tilde{p} = \mathbf{G}(\tilde{q}) \tilde{v}$.
  \STATE Compute the Jacobian determinant $J = \frac{\partial (\tilde{q},\tilde{p})}{\partial (q, p)}$ using \cref{lagrangian-remarks:eq:lagrangian-jacobian-determinant}.
  \STATE {\bf Output}: The updated position and momentum $(\tilde{q}, \tilde{p})$ and the Jacobian determinant $J$.
\end{algorithmic}
\end{algorithm}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/appendices/algorithms.tex <==
\section{Algorithms}\label{app:algorithms}

\input{algorithms/generalized-leapfrog}
\input{algorithms/lagrangian-leapfrog}
\input{algorithms/hmc}
\input{algorithms/inverted-lagrangian-leapfrog}

In this appendix we give pseudo-code implementations of algorithms featured in this work. In \cref{lagrangian-remarks:alg:generalized-leapfrog} we show the generalized leapfrog, which contrasts with the Lagrangian leapfrog in \cref{lagrangian-remarks:alg:lagrangian-leapfrog} in the presence of implicitly-defined integration steps. \Cref{lagrangian-remarks:alg:inverted-lagrangian-leapfrog} shows the Lagrangian integrator but with an inverted sequence of integration (updating position before velocity). In \cref{lagrangian-remarks:alg:hmc} we show an algorithmic implementation of a single-step of the Hamiltonian Monte Carlo Markov chain, which can be carried out using any of the integrators considered in this work.


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/appendices/involutive-monte-carlo.tex <==
\clearpage
\section{Involutive Monte Carlo}\label{lagrangian-remarks:app:involutive-monte-carlo}

\begin{proof}[Proof of \Cref{lagrangian-remarks:prop:involutive-monte-carlo-detailed-balance}]
The detailed balance condition states that for any Borel sets $(A, B), (C, D) \in \mathfrak{B}(\R^m\times\R^m)$ we have,
\begin{align}
    \int_{(A, B)} K((q, p), (C, D)) ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p =\int_{(C, D)} K((q, p), (A, B)) ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p.
\end{align}
Let $\pi(q, p)$ be the probability density on $\R^m\times\R^m$ that is proportional to $\exp(-H(q, p))$. Using the fact that $\Phi$ is an involution, it suffices to verify
\begin{align}
    &\int_{(A, B)} \alpha((q, p), \Phi(q, p), \abs{\mathrm{det}\paren{\nabla \Phi(x)}}) \mathbf{1}\set{(\tilde{q},\tilde{p})\in (C, D)} ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p \\
    =& \int_{(A, B)} \min\set{1, \frac{\pi(\Phi(q, p))}{\pi(q, p)} \abs{\mathrm{det}\paren{\nabla \Phi(x)}}} \mathbf{1}\set{\Phi(q, p)\in (C, D)} ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p \\
    =& \int_{(A, B)} \min\set{\pi(q, p), \pi(\Phi(q, p)) \abs{\mathrm{det}\paren{\nabla \Phi(x)}}} \mathbf{1}\set{\Phi(q, p)\in (C, D)} ~\mathrm{d}q~\mathrm{d}p \\
    =& \int_{(A, B)} \min\set{\frac{\pi(q, p)}{\pi(\Phi(q, p)) \abs{\mathrm{det}\paren{\nabla \Phi(x)}}}, 1} \mathbf{1}\set{\Phi(q, p)\in (C, D)} \pi(\Phi(q, p)) \abs{\mathrm{det}\paren{\nabla \Phi(x)}}~\mathrm{d}q~\mathrm{d}p \\
    =& \int_{(A, B)} \min\set{\frac{\pi(q, p)}{\pi(\Phi(q, p))} \abs{\mathrm{det}\paren{\nabla \Phi(\Phi(x))}}, 1} \mathbf{1}\set{\Phi(q, p)\in (C, D)} \pi(\Phi(q, p)) \abs{\mathrm{det}\paren{\nabla \Phi(x)}}~\mathrm{d}q~\mathrm{d}p \\
    =&  \int_{\Phi(A, B)} \min\set{1, \frac{\pi(\Phi(\tilde{q}, \tilde{p}))}{\pi(\tilde{q}, \tilde{p})} \abs{\mathrm{det}\paren{\nabla \Phi(\tilde{q}, \tilde{p})}}} \mathbf{1}\set{(\tilde{q},\tilde{p})\in (C, D)} ~\pi(\tilde{q}, \tilde{p}) ~\mathrm{d}\tilde{q}~\mathrm{d}\tilde{p} \\
    =& \int_{(C, D)} \alpha((q, p), \Phi(q, p),  \abs{\mathrm{det}\paren{\nabla \Phi(q, p)}}) \mathbf{1}\set{(q, p)\in \Phi(A, B)} ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p \\
    =& \int_{(C, D)} \alpha((q, p), \Phi(q, p),  \abs{\mathrm{det}\paren{\nabla \Phi(q, p)}}) \mathbf{1}\set{\Phi(q, p)\in (A, B)} ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p
\end{align}
Moreover, integrating over the rejection components of the transition kernel already have symmetry in $(A, B)$ and $(C, D)$:
\begin{align}
    &\int_{(A, B)} (1- \alpha((q, p), (\tilde{q}, \tilde{p}), \abs{\mathrm{det}\paren{\nabla \Phi(x)}})) \mathbf{1}\set{(q, p)\in (C, D)} ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p \\
    =& \int_{(C, D)} (1- \alpha((q, p), (\tilde{q}, \tilde{p}), \abs{\mathrm{det}\paren{\nabla \Phi(x)}})) \mathbf{1}\set{(q, p)\in (A, B)} ~\pi(q, p)~\mathrm{d}q~\mathrm{d}p.
\end{align}
Detailed balance follows as a consequence.
\end{proof}

\begin{lemma}
Let $\Phi_\epsilon : \R^m\times\R^m\to\R^m\times\R^m$ be the Lagrangian leapfrog integrator with step-size $\epsilon\in \R$. Then $\mathbf{F}\circ \Phi_\epsilon$ is an involution.
\end{lemma}
\begin{proof}
Let $(\tilde{q},\tilde{v}) = \Phi_\epsilon(q, v)$. Now we apply the Lagrangian leapfrog to $(\tilde{q},-\tilde{v})$.
\begin{align}
    \breve{v}'' &= (\mathrm{Id}_m + \Omega(\epsilon, \tilde{q}, -\tilde{v}))^{-1} \paren{-\tilde{v} - \frac{\epsilon}{2} \mathbf{G}^{-1}(\tilde{q}) \nabla U(\tilde{q})} \\
    &= -(\mathrm{Id}_m - \Omega(\epsilon, \tilde{q}, \tilde{v}))^{-1} \paren{\tilde{v} + \frac{\epsilon}{2} \mathbf{G}^{-1}(\tilde{q}) \nabla U(\tilde{q})} \\
    &= -\breve{v}
\end{align}
from \cref{lagrangian-remarks:eq:negated-i}. Moreover,
\begin{align}
    \tilde{q}'' &= \tilde{q} + \epsilon \breve{v}'' \\
    &= \tilde{q} - \epsilon \breve{v} \\
    &= q.
\end{align}
Finally,
\begin{align}
    \tilde{v}'' &= (\mathrm{Id}_m + \Omega(\epsilon, q, -\breve{v}))^{-1} \paren{-\breve{v} - \frac{\epsilon}{2} \mathbf{G}^{-1}(q) \nabla U(q)} \\
    &= -(\mathrm{Id}_m - \Omega(\epsilon, q, \breve{v}))^{-1} \paren{\breve{v} + \frac{\epsilon}{2} \mathbf{G}^{-1}(q) \nabla U(q)} \\
    &= -v
\end{align}
from \cref{lagrangian-remarks:eq:negated-ii}.
\end{proof}

==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/appendices/preliminaries.tex <==
\section{Expanded Preliminaries}

\subsection{Hamiltonian and Lagrangian Mechanics}\label{lagrangian-remarks:subsec:hamiltonian-lagrangian-mechanics}

\begin{definition}\label{lagrangian-remarks:def:hamiltonian-mechanics}
Let $H : \R^m\times\R^m\to\R$ be a smooth function, which we call the Hamiltonian. Hamilton's equations of motion are defined as the solutions to the initial value problem
\begin{align}
  \label{lagrangian-remarks:eq:hamiltonian-position} v_t &= \nabla_p H(q_t, p_t) \\
  \label{lagrangian-remarks:eq:hamiltonian-momentum} \dot{p}_t &= -\nabla_q H(q_t, p_t),
\end{align}
with $(q_0, p_0)$ a given initial position in phase space.
\end{definition}
\Cref{lagrangian-remarks:def:hamiltonian-mechanics} gives us a system of coupled first-order differential equations. Hamilton's equations of motion exhibit several key properties \citep{mechanics-and-symmetry}, which we summarize. 
\begin{theorem}\label{lagrangian-remarks:thm:hamiltonian-mechanics}
The Hamiltonian mechanics given in \cref{lagrangian-remarks:def:hamiltonian-mechanics} possess the following three properties:
\begin{enumerate}
    \item They preserve the Hamiltonian $\frac{\mathrm{d}}{\mathrm{d}t} H(q_t, p_t) = 0$.
    \item Denoting $\dot{z}_t = (v_t,\dot{p}_t)$ the equations of motion in phase space, Hamiltonian mechanics preserve volume in phase space: $\mathrm{div}(\dot{z}_t) = 0$.
    \item Under the conditions that $\nabla_q H(q, -p) = \nabla_q H(q, p)$ and $-\nabla_p H(q,p)= \nabla_pH(q, -p)$, the equations of motion are reversible via negation of the momentum variable.
\end{enumerate}
\end{theorem}
A proof is given in \cref{lagrangian-remarks:app:proofs-concerning-mechanics}.
In the special case when $U(q) = 0$ in \cref{lagrangian-remarks:eq:hamiltonian-form} for all $q\in\R^m$, Hamilton's equations of motion produce geodesic motion on the Riemannian manifold $(\R^m, \mathbf{G})$, where $\mathbf{G}$ assumes the role of the Riemannian metric \citep{Calin2004GeometricMO}.

\begin{definition}
  Given a Riemannian Hamiltonian (\cref{lagrangian-remarks:def:riemannian-hamiltonian}), define the associated {\it Lagrangian} function by,
  \begin{align}
    \label{lagrangian-remarks:eq:lagrangian-form} L(q, v) &= \tilde{K}(q, v) - U(q),
  \end{align} 
  where $\tilde{K}(q, v) = \frac{1}{2}v^\top \mathbf{G}(q) v$.
\end{definition}
Hamiltonian mechanics are related to Lagrangian dynamics by the Legendre transform which converts between momentum and velocity \citep{marsden_west_2001}.
\begin{definition}\label{lagrangian-remarks:def:legendre-transform}
  Let $L : \R^m\times\R^m\to\R$ be a Lagrangian of the form in \cref{lagrangian-remarks:eq:lagrangian-form}. The {\it Legendre transform} relates the momentum and velocity according to $p = \frac{\partial L}{\partial v}(q, v) = \mathbf{G}(q) v$. 
\end{definition}
\begin{definition}\label{lagrangian-remarks:def:inverse-legendre-transform}
  Let $H:\R^m\times\R^m\to\R$ be a Hamiltonian of the form in \cref{lagrangian-remarks:eq:hamiltonian-form}. The {\it inverse Legendre transform} relates velocity and momentum according to $v = \frac{\partial H}{\partial p}(q, p) = \mathbf{G}^{-1}(q)p$.
\end{definition}
The Lagrangian then determines equations of motion in accordance with the following physical principle.
\begin{definition}\label{lagrangian-remarks:def:hamiltons-principle}
{\it Hamilton's principle} states that the equations of motion $(q_t, v_t)$ over an interval of time $[a, b]$, with known boundary conditions $q_a$ and $q_b$, are solutions of the variational equation
\begin{align}
    \frac{\delta \mathcal{S}[q_t]}{\delta q_t} = 0
\end{align}
where
\begin{align}
    \mathcal{S}[q_t] = \int_a^b L(q_t, v_t) ~\mathrm{d}t
\end{align}
where $q_t$ and $v_t$ are related by $v_t = \frac{\mathrm{d}}{\mathrm{d}t} q_t$.
\end{definition}
Hamilton's principle states that equations of motion (as specified by $q$ and $v$) should {\it extremize} the Lagrangian subject to the boundary conditions on $q_a$ and $q_b$. 
\begin{theorem}\label{lagrangian-remarks:thm:euler-lagrange}
Under Hamilton's principle (\cref{lagrangian-remarks:def:hamiltons-principle}), the equations of motion $(q_t, v_t)$ must be solutions of the {\it Euler-Lagrange equation}
\begin{align}
  \nabla_q L(q_t, v_t) = \frac{\mathrm{d}}{\mathrm{d}t} \nabla_{v} L(q_t, v_t).
\end{align}
\end{theorem}
The equations of motion from \cref{lagrangian-remarks:thm:euler-lagrange} (or \cref{lagrangian-remarks:def:hamiltons-principle}) are, in fact, equivalent to the motion produced under Hamiltonian mechanics in \cref{lagrangian-remarks:def:hamiltonian-mechanics} \citep{mechanics-and-symmetry}. For Lagrangians of the form in \cref{lagrangian-remarks:eq:lagrangian-form}, the $k$-th element of the acceleration is,
\begin{align}
  \label{lagrangian-remarks:eq:lagrangian-acceleration} a_t^{(k)} = -\sum_{i=1}^m\sum_{j=1}^m \Gamma^k_{ij}(q_t) v_t^{(i)} v_t^{(j)} - \sum_{l=1}^m \mathbf{G}^{-1}_{kl}(q_t) \frac{\partial U}{\partial q^{(l)}} (q_t),
\end{align}
where $\Gamma^k_{ij}$ are the Christoffel symbols (\cref{lagrangian-remarks:def:christoffel-symbols}).
We conclude this section by noting that $\Omega$ in \cref{lagrangian-remarks:eq:omega} enjoys the following properties:
\begin{proposition}\label{lagrangian-remarks:prop:omega-properties}
The function $\Omega : \R\times\R^m\times\R^m\to\R^{m\times m}$ in \cref{lagrangian-remarks:eq:omega} satisfies 
  \begin{align}
      \label{lagrangian-remarks:eq:omega-symmetry} \Omega(\epsilon, q, v)\breve{v} &= \Omega(\epsilon, q, \breve{v}) v \\
      \label{lagrangian-remarks:eq:omega-derivative} \frac{\partial}{\partial v} (\Omega(\epsilon, q, v)\breve{v}) &= \Omega(\epsilon, q, \breve{v}).
  \end{align}
\end{proposition}
\begin{proof}
The result in \cref{lagrangian-remarks:eq:omega-symmetry} can be seen from
\begin{align}
    (\Omega(\epsilon, q, v)\breve{v})_i &= \frac{\epsilon}{2} \sum_{j=1}^m \sum_{k=1}^m \Gamma^i_{kj}(q) v^{(k)} \breve{v}^{(j)} \\
    &= \frac{\epsilon}{2} \sum_{j=1}^m \sum_{k=1}^m \Gamma^i_{jk}(q) v^{(k)} \breve{v}^{(j)} \\
    &= \frac{\epsilon}{2} \sum_{k=1}^m \sum_{j=1}^m \Gamma^i_{jk}(q) v^{(k)} \breve{v}^{(j)} \\
    &= (\Omega(\epsilon, q, \breve{v})v)_i.
\end{align}
\Cref{lagrangian-remarks:eq:omega-derivative} then follows as an immediate corollary.
\end{proof}
Like Hamiltonian mechanics, Lagrangian dynamics conserve the Hamiltonian (when $p_t = \mathbf{G}(q_t) v_t$) and are reversible. However, Lagrangian dynamics do not conserve volume in $(q, v)$-space.


\subsection{Background on Numerical Integrators}\label{lagrangian-remarks:subsec:numerical-integrators}


The Hamiltonian equations of motion in \cref{lagrangian-remarks:eq:hamiltonian-position,lagrangian-remarks:eq:hamiltonian-momentum} and the Lagrangian motion described in \cref{lagrangian-remarks:eq:lagrangian-acceleration} rarely have closed-form solutions. Therefore, it is necessary to investigate methods of numerical integration to produce approximate solutions to these initial value problems. In the following section, we review key ideas from \citet{Hairer:1250576}.
\begin{definition}\label{lagrangian-remarks:def:initial-value-problem}
  Let $g : \R^m\to\R^m$. {\it The solution to an initial value problem} is a function $z_{(\cdot)} : \R\to\R^m$ for which $\frac{\mathrm{d}}{\mathrm{d}t} z_t = g(z_t)$ and for which the {\it initial value} $z_0\in\R^m$ is known. In this case $g$ is called a {\it (time-homogenous) vector field}.
\end{definition}
\begin{definition}\label{lagrangian-remarks:def:integrator-order}
  Let $z_t$ be the solution to an initial value problem (\cref{lagrangian-remarks:def:initial-value-problem}) with initial value $z_0$. A {\it numerical integrator with step-size $\epsilon$} is a mapping $\Phi_{\epsilon} : \R^m\to\R^m$ and is said to have order $p$ if $\Vert \Phi_{\epsilon}(z_0) - z_{\epsilon}\Vert = \mathcal{O}(\epsilon^{p+1})$.
\end{definition}
\begin{definition}\label{lagrangian-remarks:def:self-adjoint}
  The adjoint of a numerical method $\Phi_\epsilon : \R^m \to\R^m$ is defined by the relation $\Phi_\epsilon^*(z) = \Phi^{-1}_{-\epsilon}(z)$. The numerical method $\Phi_\epsilon$ is said to be self-adjoint if $\Phi^*_\epsilon = \Phi_\epsilon$.
\end{definition}
\begin{theorem}[\citet{Hairer:1250576}]\label{lagrangian-remarks:thm:self-adjoint-even-order}
  Consider an initial value problem $\dot{z}_t = g(z_t)$ with initial condition $z_0 \in \R^m$. Let $\Phi_\epsilon$ be a one-step numerical integrator of (maximal) order $r\in\mathbb{N}$. If $\Phi_\epsilon$ is self-adjoint, then $r$ is even.
\end{theorem}
\begin{proposition}\label{lagrangian-remarks:prop:composition-order}
Let $g : \R^m\to\R^m$ be a time-homogenous vector field. Let $\Xi:\R^m\to\R^m$ be a diffeomorphism. Let $z_t$ be the solution to the initial value problem $\dot{z}_t = g(z_t)$ given $z_0$. Let $\Phi_\epsilon : \R^m\to\R^m$ be the flow map of $z_\epsilon$ and suppose that $\hat{\Phi}_\epsilon$ is a $p$-th order approximation of $\Phi_\epsilon$. Then $\Xi\circ \hat{\Phi}_\epsilon$ is a $p$-th order approximation of $\Xi\circ \Phi_\epsilon$.
\end{proposition}
A proof is given in \cref{lagrangian-remarks:app:proofs-concerning-numerical-order}.

\begin{proposition}
  The generalized leapfrog integrator is a second-order (\cref{lagrangian-remarks:def:integrator-order}), self-adjoint (\cref{lagrangian-remarks:def:self-adjoint}) numerical method.
\end{proposition}



\subsection{Hamiltonian and Lagrangian Monte Carlo}\label{lagrangian-remarks:subsec:hamiltonian-lagrangian-monte-carlo}


Our objective in Bayesian inference is to draw samples from the distribution whose density is $\pi(q) \propto \exp(\mathcal{L}(q))$. We now review basic concepts from Markov chain Monte Carlo.
\begin{definition}
  A {\it Markov chain transition kernel} is a map $K : \R^m\times\mathfrak{B}(\R^m) \to [0,1]$ satisfying (i) for every $x\in \R^m$ the map $A\mapsto K(x, A)$ is a probability measure and (ii) for every $A \in\mathfrak{B}(\R^m)$, the map $x\mapsto K(x, A)$ is measurable. Given a Markov chain transition kernel $K$, a {\it Markov chain} is defined inductively by $x_{n+1} \vert x_n \sim K(x_n, \cdot)$.
\end{definition}
HMC accomplishes this by artificially expanding the distribution to incorporate a momentum variable. Defining $U(q) = -\mathcal{L}(q) + \frac{1}{2} \log\mathrm{det}(\mathbf{G}(q))$, let $H(q, p)$ be the Hamiltonian given in \cref{lagrangian-remarks:eq:hamiltonian-form} and observe that the density $\pi(q, p) \propto \exp(-H(q, p))$ has $\pi(q) = \int_{\R^m} \pi(q, p) ~\mathrm{d}p$ and $p \vert q \sim\mathrm{Normal}(0, \mathbf{G}(q))$. In order to unify methods of Bayesian inference based on either the generalized leapfrog integrator (\cref{lagrangian-remarks:def:generalized-leapfrog}) or the Lagrangian leapfrog (\cref{lagrangian-remarks:def:lagrangian-leapfrog}) under one framework, we now introduce the Markov chain transition kernel based on smooth involutions.
\begin{definition}[\citet{DBLP:conf/icml/NeklyudovWEV20}]\label{lagrangian-remarks:def:involutive-monte-carlo}
  Let $\Phi : \R^m\times\R^m\to\R^m\times\R^m$ be a smooth involution (i.e. $\Phi=\Phi^{-1}$). Let $\pi:\R^m\times\R^m\to\R_+$ be a probability density with respect to Lebesgue measure. Then we define the Markov chain transition kernel of {\it involutive Monte Carlo} by
  \begin{align}
  \begin{split}
      K((q, p), (A, B)) &= \alpha((q, p), (\tilde{q},\tilde{p}), J)~\mathbf{1}\set{(\tilde{q}, \tilde{p})\in (A, B)} \\
      &\qquad + \paren{1-\alpha((q, p), (\tilde{q},\tilde{p}), J)} ~\mathbf{1}\set{(q, p)\in (A, B)}
  \end{split} \\
  \label{lagrangian-remarks:eq:acceptance-probability} \alpha((q, p), (\tilde{q}, \tilde{p}), J) &= \min\set{1, \frac{\exp(-H(\tilde{q}, \tilde{p}))}{\exp(-H(q, p))}\cdot J} \\
  J &= \abs{\mathrm{det}\paren{\frac{\partial (\tilde{q}, \tilde{p})}{\partial (q, p)}}},
  \end{align}
  where $(A, B)\in\mathfrak{B}(\R^m\times\R^m)$ and $(\tilde{q}, \tilde{p}) = \Phi(q, p)$.
\end{definition}
\begin{proposition}\label{lagrangian-remarks:prop:involutive-monte-carlo-detailed-balance}
  The Markov chain transition kernel of involutive Monte Carlo satisfies detailed balance with respect to the distribution whose density is $\pi(q, p)\propto \exp(-H(q, p))$.
\end{proposition}
A proof is provided in \cref{lagrangian-remarks:app:involutive-monte-carlo}. Central to the construction of involutions of interest to us is the momentum flip operator, defined as follows.
\begin{definition}\label{lagrangian-remarks:def:momentum-flip}
  The {\it momentum flip operator} is the map $\mathbf{F}(q, p) = (q, -p)$.
\end{definition}
The fact that numerical integrators can be combined with the momentum flip operator in order to produce involutions is covered in \cref{lagrangian-remarks:app:involutive-monte-carlo} in the case of the Lagrangian leapfrog; other integrators are handled similarly.
We provide pseudo-code implementing a single step of involutive Monte Carlo in \cref{lagrangian-remarks:alg:hmc} with involutions provided by the generalized leapfrog or Lagrangian leapfrog integrator. Given an initial point $(q_0, p_0)$ in phase space drawn from the distribution $\pi(q, p)$, the sequence of states $((q_1,p_1), (q_2, p_2), \ldots)$ computed by \cref{lagrangian-remarks:alg:hmc} are guaranteed to have $\pi(q, p)$ as their marginal distributions. Under the additional conditions that the HMC Markov chain is irreducible and aperiodic, HMC also produces an ergodic chain. 

The generalized leapfrog integrator is volume preserving. However, the integrator of Lagrangian dynamics is not. The required change-of-volume can be deduced as follows. First, observe that the update \cref{lagrangian-remarks:eq:lagrangian-position-update} is immediately volume-preserving since it is merely the translation of the position variable by a quantity. The change of volume incurred in \cref{lagrangian-remarks:eq:lagrangian-velocity-i} has a Jacobian determinant given by,
\begin{align}
  \abs{\mathrm{det}\paren{\frac{\partial (q, \breve{v})}{\partial (q, v)}}} = \abs{\frac{\mathrm{det}(\mathrm{Id}_m - \Omega(\epsilon, q, \breve{v}))}{\mathrm{det}(\mathrm{Id}_m + \Omega(\epsilon, q, v))}}.
\end{align}
The update in \cref{lagrangian-remarks:eq:lagrangian-velocity-ii} incurs a similar change of volume. Thus, when employing \cref{lagrangian-remarks:alg:lagrangian-leapfrog}, the Jacobian determinant of the transformation $(q, p)\mapsto (\tilde{q}, \tilde{p})$ is,
\begin{align}
  \begin{split}
    \label{lagrangian-remarks:eq:lagrangian-jacobian-determinant} &\abs{\mathrm{det}\paren{\frac{\partial (\tilde{q}, \tilde{p})}{\partial (q, p)}}} = \mathrm{det}(\mathbf{G}^{-1}(q))\mathrm{det}(\mathbf{G}(\tilde{q})) ~\times \\
    &\qquad \abs{\frac{\mathrm{det}(\mathrm{Id}_m - \Omega(\epsilon, \tilde{q}, \tilde{v})) \mathrm{det}(\mathrm{Id}_m - \Omega(\epsilon, q, \breve{v}))}{\mathrm{det}(\mathrm{Id}_m + \Omega(\epsilon, \tilde{q}, \breve{v})) \mathrm{det}(\mathrm{Id}_m + \Omega(\epsilon, q, v))}}.
  \end{split}
\end{align}
\begin{definition}\label{lagrangian-remarks:def:rmhmc}
  Let $\Phi_\epsilon$ be the generalized leapfrog integrator with step-size $\epsilon\in\R$ (\cref{lagrangian-remarks:def:generalized-leapfrog}). Let $k\in\mathbb{N}$ be a number of integration steps. The {\it Riemannian manifold Hamiltonian Monte Carlo (RMHMC) Markov chain} is an instance involutive Monte Carlo (\cref{lagrangian-remarks:def:involutive-monte-carlo}) with involution $\mathbf{F} \circ \Phi_{\epsilon}^k$.
\end{definition}
\begin{definition}\label{lagrangian-remarks:def:lmc}
  Let $\Phi_\epsilon$ be the Lagrangian leapfrog integrator with step-size $\epsilon\in\R$ (\cref{lagrangian-remarks:def:lagrangian-leapfrog}). Let $k\in\mathbb{N}$ be a number of integration steps. The {\it Lagrangian Monte Carlo (LMC) Markov chain} is an instance involutive Monte Carlo (\cref{lagrangian-remarks:def:involutive-monte-carlo}) with involution $\mathbf{F} \circ \Phi_{\epsilon}^k$.
\end{definition}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/appendices/proofs-concerning-mechanics.tex <==
\section{Proofs Concerning Mechanics Systems}\label{lagrangian-remarks:app:proofs-concerning-mechanics}

We give a proof of \cref{lagrangian-remarks:thm:hamiltonian-mechanics}.
\begin{proof}
We first show that the Hamiltonian energy is conserved. 
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} H(q_t, p_t) &= \nabla_q H(q_t, p_t) \cdot v_t + \nabla_p H(q_t, p_t) \cdot \dot{p}_t \\
    &= \nabla_q H(q_t, p_t) \cdot \nabla_p H(q_t, p_t) - \nabla_p H(q_t, p_t) \cdot \nabla_q H(q_t, p_t) \\
    &= 0.
\end{align}
Next we show that Hamiltonian mechanics conserve volume in $(q, p)$-space. This is equivalent to the vector field $(v_t, \dot{p}_t)$ having zero divergence, which we now verify.
\begin{align}
    \mathrm{div}(v_t, \dot{p}_t) &= \nabla_q \cdot v_t + \nabla_p \cdot \dot{p}_t \\
    &= \nabla_q \cdot \nabla_p H(q_t, p_t) - \nabla_p \cdot \nabla_q H(q_t, p_t) \\
    &= \sum_{i=1}^m \frac{\partial^2 H}{\partial q_i \partial p_i} H(q_t, p_t) - \sum_{i=1}^m \frac{\partial^2 H}{\partial p_i \partial q_i} H(q_t, p_t) \\
    &= 0,
\end{align}
by symmetry of partial derivatives. Finally we show that under the conditions that $\nabla_q H(q, -p) = \nabla_q H(q, p)$ and $\nabla_p H(q, -p) = -\nabla_p H(q, p)$ that the equations of motion are reversible under negation of the momentum variable. To see this, fix $\tau \in \R_+$ and consider $(q_t, p_t)$ satisfying \cref{lagrangian-remarks:eq:hamiltonian-position,lagrangian-remarks:eq:hamiltonian-momentum} for $t\in [0, \tau]$. Let $\tilde{p}_t = -p_{\tau-t}$ and $\tilde{q}_t = q_{\tau-t}$. We find that $\tilde{q}_t$ and $\tilde{p}_t$ obey the following equations of motion:
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} \tilde{q}_t &= -v_{\tau-t} \\
    &= -\nabla_p H(q_{\tau-t}, p_{\tau-t}) \\
    &= \nabla_p H(\tilde{q}_t, -p_{\tau-t}) \\
    &= \nabla_p H(\tilde{q}_t, \tilde{p}_{t}) \\
    \frac{\mathrm{d}}{\mathrm{d}t} \tilde{p}_t &= \dot{p}_{\tau-t} \\
    &= -\nabla_q H(q_{\tau-t}, p_{\tau-t}) \\
    &= -\nabla_q H(q_{\tau-t}, -p_{\tau-t}) \\
    &= -\nabla_q H(\tilde{q}_t, \tilde{p}_t).
\end{align}
Thus we see that $(\tilde{q}_t, \tilde{p}_t)$ are also solutions to Hamilton's equations of motion and satisfy $\tilde{q}_\tau = q_0$ and $\tilde{p}_\tau = -p_0$, demonstrating reversibility.
\end{proof}

==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/appendices/proofs-concerning-numerical-order.tex <==
\clearpage
\section{Proofs Concerning the Numerical Order of the Lagrangian Integrators}\label{lagrangian-remarks:app:proofs-concerning-numerical-order}

The claim of first order accuracy was derived in \citet{lan2015}; we have included a proof for completeness.
\begin{proof}[Proof of \cref{lagrangian-remarks:lem:second-order-local-error}]
Let $q_t$ and $v_t$ be solutions to the initial value problem,
\begin{align}
    \dot{q}_t &= v_t \\
    \dot{v}_t &= -\Omega(2, q_t, v_t) v_t - \mathbf{G}^{-1}(q_t) \nabla U(q_t).
\end{align}
Given the initial value $q_0 = q$ and $v_0 = v$, we can expand the solution in a Taylor series about $t=0$.
\begin{align}
    q_t &= q_0 + t \dot{q}_0 + \mathcal{O}(t^2) \\
    &= q + t v + \mathcal{O}(t^2) \\
    v_t &= v_0 - t \paren{\Omega(2, q_0, v_0) v_0 - \mathbf{G}^{-1}(q_0) \nabla U(q_0)} + \mathcal{O}(t^2) \\
    &= v - \Omega(2t, q, v) v - t \mathbf{G}^{-1}(q) \nabla U(q) + \mathcal{O}(t^2).
\end{align}
Letting $t=\epsilon$ gives the following approximations,
\begin{align}
    q_{\epsilon} &= q + \epsilon v + \mathcal{O}(\epsilon^2) \\
    v_{\epsilon} &= v - \Omega(2\epsilon, q, v) v - \epsilon \mathbf{G}^{-1}(q) \nabla U(q) + \mathcal{O}(\epsilon^2)
\end{align}
Now we expand the steps of the explicit numerical integrator. We begin with the first update to velocity.
\begin{align}
\breve{v} &= \paren{\mathrm{Id}_m + \Omega(\epsilon, q, v)}^{-1} \paren{v - \frac{\epsilon}{2} \mathbf{G}^{-1}(q)\nabla U(q)} \\
&= \paren{\mathrm{Id}_m - \Omega(\epsilon, q, v) + \mathcal{O}(\epsilon^2)}\paren{v - \frac{\epsilon}{2} \mathbf{G}^{-1}(q)\nabla U(q)} \\
&= v - \Omega(\epsilon, q, v) v - \frac{\epsilon}{2} \mathbf{G}^{-1}(q) \nabla U(q) + \mathcal{O}(\epsilon^2)
\end{align}
Now we expand the update to position.
\begin{align}
\tilde{q} &= q + \epsilon \breve{v} \\
&= q + \epsilon v + \mathcal{O}(\epsilon^2)
\end{align}
We conclude by expanding the second update to velocity in terms of the initial conditions.
\begin{align}
\tilde{v} &= \paren{\mathrm{Id}_m + \Omega(\epsilon, \tilde{q}, \breve{v})}^{-1} \paren{\breve{v} - \frac{\epsilon}{2} \mathbf{G}^{-1}(\tilde{q})\nabla U(\tilde{q})} \\
&= \breve{v} - \Omega(\epsilon, \tilde{q}, \breve{v}) \breve{v} - \frac{\epsilon}{2} \mathbf{G}^{-1}(\tilde{q}) \nabla U(\tilde{q}) + \mathcal{O}(\epsilon^2) \\
&= \breve{v} - \Omega(\epsilon, q, v) v - \frac{\epsilon}{2} \mathbf{G}^{-1}(q) \nabla U(q) + \mathcal{O}(\epsilon^2) \\
&= v - \Omega(2\epsilon, q, v) v - \epsilon \mathbf{G}^{-1}(q) \nabla U(q) + \mathcal{O}(\epsilon^2).
\end{align}
Therefore, a single step of the numerical integrator with step-size $\epsilon$ agrees with the analytical solution to the initial value problem (from the same initial condition) to at least first order in $\epsilon$.
\end{proof}

\begin{proof}[Proof of \Cref{lagrangian-remarks:lem:inverted-lagrangian-properties}]
To demonstrate that the inverted integrator has at least first-order error, we expand the steps of the integrator as follows. First,
\begin{align}
    \breve{q} &= q + \frac{\epsilon}{2} ~v \\
    \tilde{v} &= \paren{\mathrm{Id}_m + \Omega(2\epsilon, \breve{q}, v)}^{-1} \paren{v - \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q})} \\
    &= \paren{\mathrm{Id}_m + \Omega(2\epsilon, \breve{q}, v)} \paren{v - \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q})} + \mathcal{O}(\epsilon^2) \\
    &= v - \Omega(2\epsilon, q, v) v - \epsilon \mathbf{G}^{-1}(q) \nabla U(q) + \mathcal{O}(\epsilon^2) \\
    \tilde{q} &= \breve{q} + \frac{\epsilon}{2} \tilde{v} \\
    &= q + \frac{\epsilon}{2} ~v + \frac{\epsilon}{2} ~v + \mathcal{O}(\epsilon^2) \\
    &= q + \epsilon ~v.
\end{align}
This verifies that the inverted Lagrangian leapfrog has at least first order accuracy. 

In order to show that the inverted leapfrog integrator is symmetric, we proceed as follows. Recall that the three steps of the inverted Lagrangian leapfrog are
\begin{align}
    \breve{q} &= q + \frac{\epsilon}{2} ~v \\
    \tilde{v} &= \paren{\mathrm{Id}_m + \Omega(2\epsilon, \breve{q}, v)}^{-1} \paren{v - \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q})} \\
    \tilde{q} &= \breve{q} + \frac{\epsilon}{2} ~\tilde{v}.
\end{align}
Therefore, we consider integrating from initial position $(\tilde{q},\tilde{v})$ with a negated step-size $-\epsilon$ as follows:
\begin{align}
    \breve{q}' &= \tilde{q} - \frac{\epsilon}{2} ~\tilde{v} \\
    &= \breve{q}
\end{align}
For the velocity we have,
\begin{align}
    & \tilde{v}' = \paren{\mathrm{Id}_m - \Omega(2\epsilon, \breve{q}, \tilde{v})}^{-1} \paren{\tilde{v} + \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q})} \\
    \implies& \paren{\mathrm{Id}_m - \Omega(2\epsilon, \breve{q}, \tilde{v})} \tilde{v}' = \tilde{v} + \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q}) \\
    \implies& \tilde{v} + \Omega(2\epsilon, \breve{q}, \tilde{v}')\tilde{v} = \tilde{v}' - \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q}) \\
    \implies& \tilde{v} = \paren{\mathrm{Id}_m + \Omega(2\epsilon, \breve{q}, \tilde{v}'}^{-1} \paren{\tilde{v}' - \epsilon \mathbf{G}^{-1}(\breve{q})\nabla U(\breve{q})} \\
    \implies \tilde{v}' = v
\end{align}
Finally, the last update to the position is,
\begin{align}
    \tilde{q}' &= \breve{q} - \frac{\epsilon}{2} v \\
    &= q.
\end{align}
Hence we see that the inverted Lagrangian leapfrog is also self-adjoint. As noted in the main text, the combination of self-adjointness and at least first-order accuracy immediately imply second-order accuracy.
\end{proof}

\begin{proof}[Proof of \cref{lagrangian-remarks:lem:self-adjoint}]
Self-adjointness of a numerical integrator follows immediately from the condition $\Phi_{-\epsilon}\circ \Phi_{\epsilon} = \mathrm{Id}$. Therefore, to demonstrate that a numerical method is self-adjoint it suffices to establish this condition. Consider the first update to the velocity:
\begin{align}
    &\breve{v} = \paren{\mathrm{Id}_m + \Omega(\epsilon, q, v)}^{-1}\paren{v - \frac{\epsilon}{2} \mathbf{G}(q)^{-1}\nabla U(q)} \\
    \iff& \breve{v} + \Omega(\epsilon, q, v) \breve{v} = v - \frac{\epsilon}{2} \mathbf{G}(q)^{-1} \nabla U(q) \\
    \iff & \breve{v} + \frac{\epsilon}{2} \mathbf{G}(q)^{-1} \nabla U(q) = v - \Omega(\epsilon, q, \breve{v}) v \\
    \iff &  \breve{v} + \frac{\epsilon}{2} \mathbf{G}(q)^{-1} \nabla U(q) = \paren{\mathrm{Id}_m - \Omega(\epsilon, q, \breve{v})} v \\
    \iff & v = \paren{\mathrm{Id}_m - \Omega(\epsilon, q, \breve{v})}^{-1}\paren{\breve{v} + \frac{\epsilon}{2} \mathbf{G}^{-1}(q)\nabla U(q)}.
\end{align}
An identical series of computations reveals,
\begin{align}
    \breve{v} = \paren{\mathrm{Id}_m - \Omega(\epsilon, \tilde{q}, \tilde{v})}^{-1}\paren{\tilde{v} + \frac{\epsilon}{2} \mathbf{G}^{-1}(\tilde{q})\nabla U(\tilde{q})}.
\end{align}
Hence, applying $\Phi_{-\epsilon}$ to $(\tilde{q}, \tilde{v})$ yields the following series of updates,
\begin{align}
    \label{lagrangian-remarks:eq:negated-i} \breve{v}' &= \paren{\mathrm{Id}_m - \Omega(\epsilon, \tilde{q}, \tilde{v})}^{-1}\paren{\tilde{v} + \frac{\epsilon}{2} \mathbf{G}^{-1}(\tilde{q})\nabla U(\tilde{q})} \\
    &= \breve{v} \\
    q' &= \tilde{q} - \epsilon \breve{v}' \\
    &= \tilde{q} - \epsilon \breve{v} \\
    &= q \\
    \label{lagrangian-remarks:eq:negated-ii} v' &= \paren{\mathrm{Id}_m - \Omega(\epsilon, q, \breve{v})}^{-1}\paren{\breve{v} + \frac{\epsilon}{2} \mathbf{G}^{-1}(q)\nabla U(q)} \\
    &= v.
\end{align}
Hence we return to the initial condition $(q, v)$. This verifies that the explicit integrator employed in LMC is self-adjoint.
\end{proof}


\begin{proof}[Proof of \Cref{lagrangian-remarks:prop:composition-order}]
Since $\hat{\Phi}_\epsilon$ is $p$-th order accurate for $\Phi_\epsilon$ we have, by Taylor series expansion, that,
\begin{align}
    \label{eq:2021-12-19-taylor-i} \hat{\Phi}_0 &= \Phi_0 \\
    \label{eq:2021-12-19-taylor-ii} \frac{\mathrm{d}^k}{\mathrm{d}\epsilon^k} \hat{\Phi}_\epsilon(z_0) \bigg|_{\epsilon=0} &= \frac{\mathrm{d}^k}{\mathrm{d}\epsilon^k} \Phi_\epsilon(z_0) \bigg|_{\epsilon=0},
\end{align}
for $k=1,\ldots, p$. Let $f : \R\to\R^m$, then the Taylor series of expansion of $\Xi\circ f(\epsilon)$ is,
\begin{align}
    \label{eq:2021-12-19-taylor-composition} \Xi \circ f(\epsilon) &= \Xi\circ f(0) + \sum_{k=1}^p \epsilon^k g^{[k]}\paren{f(0), \frac{\mathrm{d}}{\mathrm{d}\epsilon} f(0), \ldots, \frac{\mathrm{d}^k}{\mathrm{d}\epsilon^k} f(0)} + \mathcal{O}(\epsilon^{p+1}),
\end{align}
where $g^{[k]}$ are functions determining the Taylor series coefficients which depend on the derivatives of $f$. For instance,
\begin{align}
    g^{[1]}\paren{f(0), \frac{\mathrm{d}}{\mathrm{d}\epsilon} f(0)} &= \nabla \Xi(f(0)) \cdot \frac{\mathrm{d}}{\mathrm{d}\epsilon} f(0) \\
    g^{[2]}\paren{f(0), \frac{\mathrm{d}}{\mathrm{d}\epsilon} f(0), \frac{\mathrm{d}^2}{\mathrm{d}\epsilon^2} f(0)} &= \nabla^2 \Xi(f(0))\paren{\frac{\mathrm{d}}{\mathrm{d}\epsilon} f(0), \frac{\mathrm{d}}{\mathrm{d}\epsilon} f(0)} + \nabla\Xi(f(0)) \cdot \frac{\mathrm{d}^2}{\mathrm{d}\epsilon^2} f(0).
\end{align}
By the equality of the Taylor series expansion coefficients in \cref{eq:2021-12-19-taylor-i,eq:2021-12-19-taylor-ii} it follows from \cref{eq:2021-12-19-taylor-composition} that,
\begin{align}
    \Xi\circ\Phi_\epsilon(z_0) - \Xi\circ\hat{\Phi}_\epsilon(z_0) = \mathcal{O}(\epsilon^{p+1}).
\end{align}
This proves that $\Xi\circ\hat{\Phi}_\epsilon$ is also $p$-th order accurate for $\Xi\circ\Phi_\epsilon$.
\end{proof}

==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/appendices/propagator-matrices.tex <==
\clearpage
\section{Propagator Matrices for the Leapfrog and Inverted Leapfrog}\label{lagrangian-remarks:app:propagator-matrices}

\begin{definition}\label{lagrangian-remarks:def:standard-leapfrog}
  The {\it generalized leapfrog integrator} for the Hamiltonian equations of motion in \cref{lagrangian-remarks:eq:hamiltonian-position,lagrangian-remarks:eq:hamiltonian-momentum} with Hamiltonian $H(q, p) = U(q) + p^\top p / 2$ is a map $(q, p)\mapsto (\tilde{q}, \tilde{p})$ defined by,
  \begin{align}
  \breve{p} &= p - \frac{\epsilon}{2} \nabla U(q) \\
  \tilde{q} &= q + \epsilon ~\breve{p} \\
  \tilde{p} &= \breve{p} - \frac{\epsilon}{2} \nabla U(\tilde{q}).
  \end{align}
\end{definition}
\begin{definition}\label{lagrangian-remarks:def:inverted-leapfrog}
  The {\it generalized leapfrog integrator} for the Hamiltonian equations of motion in \cref{lagrangian-remarks:eq:hamiltonian-position,lagrangian-remarks:eq:hamiltonian-momentum} with Hamiltonian $H(q, p) = U(q) + p^\top p / 2$ is a map $(q, p)\mapsto (\tilde{q}, \tilde{p})$ defined by,
  \begin{align}
  \breve{q} &= q + \frac{\epsilon}{2} p \\
  \tilde{p} &= p - \epsilon \nabla U(q) \\
  \tilde{q} &= \breve{q} + \frac{\epsilon}{2} \tilde{p}.
  \end{align}
\end{definition}

For Hamiltonians of the form $H(q, p) = \omega^2 q^2 / 2 + p^2 / 2$, the action of the leapfrog and inverted leapfrog integrators are linear. This means that there are matrices, called ``propagator matrices,'' which, when acting on the vector $(q, p)\in\R^2$, produce the same position in phase space as the integrators themselves. Computing integer matrix powers of these matrices can then produce the multi-step output of the integrators. In the case of the leapfrog integrator, the propagator matrix is \citep{leimkuhler_reich_2005},
\begin{align}
  \begin{pmatrix} \tilde{q} \\ \tilde{p} \end{pmatrix} = \underbrace{\begin{pmatrix} 1 - \frac{\epsilon^2\omega^2}{2} & \epsilon \\ \epsilon\omega^2\paren{1 - \frac{\epsilon^2\omega^2}{4}} & 1 - \frac{\epsilon^2\omega^2}{2} \end{pmatrix}}_{\mathbf{R}'} \begin{pmatrix} q \\ p \end{pmatrix}.
\end{align}
The propagator matrix for the inverted leapfrog is,
\begin{align}
  \begin{pmatrix} \tilde{q} \\ \tilde{p} \end{pmatrix} = \underbrace{\begin{pmatrix} 1 - \frac{\epsilon^2\omega^2}{2} & \epsilon\paren{1 - \frac{\epsilon^2\omega^2}{4}} \\ -\epsilon\omega^2 & 1 - \frac{\epsilon^2\omega^2}{2} \end{pmatrix}}_{\mathbf{R}''} \begin{pmatrix} q \\ p \end{pmatrix}.
\end{align}
At stationarity,
\begin{align}
  \begin{pmatrix} q \\ p \end{pmatrix} \sim \mathrm{Normal}\paren{\begin{pmatrix} 0 \\ 0 \end{pmatrix}, \begin{pmatrix} 1 / \omega^2 & 0 \\ 0 & 1 \end{pmatrix}}.
\end{align}
Therefore, for an integrator with propagator matrix $\mathbf{R}$, the distribution of the $k$-step transition is,
\begin{align}
  \mathrm{Normal}\paren{\begin{pmatrix} 0 \\ 0 \end{pmatrix}, \mathbf{R}^k\begin{pmatrix} 1 / \omega^2 & 0 \\ 0 & 1 \end{pmatrix} (\mathbf{R}^k)^\top},
\end{align}



==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/banana/banana.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/banana/esjd.png}
  \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/banana/ess-per-second.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/banana/ks.png}
  \caption{Kolmogorov-Smirnov}
  \end{subfigure}
  \caption{{\bf (Banana-Shaped Distribution)} We show the ESJD, the minimum ESS per second, and the distribution of Kolmogorov-Smirnov statistics for sampling from the banana-shaped distribution using RMHMC, LMC, and ILMC. Surprisingly, we do not observe degradation of the ESJD when employing ILMC. Therefore, combined with its faster sampling iteration, ILMC enjoys the best ESS per second and a distribution of Kolmogorov-Smirnov statistics that is comparable to LMC.}
  \label{lagrangian-remarks:fig:banana}
\end{figure*}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/fitzhugh-nagumo/fitzhugh-nagumo.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/ess-per-second-True.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/ks-True.png}
  \caption{Kolmogorov-Smirnov}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/fitzhugh-nagumo/ks-False.png}
  \caption{Kolmogorov-Smirnov (Misspecified)}
  \end{subfigure}
  \caption{{\bf (Fitzhugh-Nagumo Model)} We show the minimum ESS per second and the Kolmogorov-Smirnov ergodicity metric for inferring the posterior distribution of $(a, b,c)$ in the Fitzhugh-Nagumo posterior distribution. We observe that LMC has the strongest performance in terms of time-normalized ESS and that all methods exhibit comparable performance with respect to ergodicity. When we break the symmetry of partial derivatives, RMHMC no longer has the target distribution as its invariant distribution; this causes a degradation of the ergodicity metric. However, the geometric methods LMC and ILMC are robust to this misspecification because they are non-volume-preserving by design.}
  \label{lagrangian-remarks:fig:fitzhugh-nagumo}
\end{figure*}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/logistic-regression/logistic-breast.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/logistic/breast-cancer-esjd.png}
  \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/logistic/breast-cancer-min-ess-per-second.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/logistic/breast-cancer-mean-ess-per-second.png}
  \caption{Mean ESS / Sec.}
  \end{subfigure}
  \caption{{\bf (Logistic Regression - Breast Cancer)} We show the ESJD and the minimum and mean ESS per second for the breast cancer dataset using RMHMC, LMC, and ILMC. We observe that LMC and ILMC have degraded movement through the sample space as computed by the ESJD; however, this is compensated for by their superior computational efficiency, ultimately yielding more effectively independent samples per second and RMHMC.}
  \label{lagrangian-remarks:fig:logistic-breast}
\end{figure*}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/logistic-regression/logistic-thyroid.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/logistic/thyroid-esjd.png}
  \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/logistic/thyroid-min-ess-per-second.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/logistic/thyroid-mean-ess-per-second.png}
  \caption{Mean ESS / Sec.}
  \end{subfigure}
  \caption{{\bf (Logistic Regression - Thyroid Cancer)} We show the ESJD and the minimum and mean ESS per second for the thyroid cancer dataset using RMHMC, LMC, and ILMC. We observe that LMC and ILMC have significantly degraded movement through the sample space as computed by the ESJD; however, this is compensated for by their superior computational efficiency, ultimately yielding more effectively independent samples per second and RMHMC.}
  \label{lagrangian-remarks:fig:logistic-thyroid}
\end{figure*}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/position-difference.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{images/ess-reduction/expected-squared-distance.png}
  \caption{Visualization of the difference in expected distance when integrating a trajectory of a separable, quadratic Hamiltonian for a varying number of steps and integration step-sizes. This difference is always non-negative, indicating that one expects a greater distance between position variables when integrating with the leapfrog, rather than inverted leapfrog, algorithm.}
  \label{lagrangian-remarks:fig:position-difference}
\end{figure}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/second-order.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{images/second-order/non-separable-second-order.png}
  \caption{Visualization of the second-order accuracy (i.e. third order local error) of the Lagrangian integrator on Lagrangian dynamics derived from a non-separable Hamiltonian. We see that the observed local error decreases on a log-log scale with a slope of three, corresponding to the claimed third-order local error. By contrast, we also show a line with a slope of two, indicating that the integrator exhibits accuracy better than first-order.}
  \label{lagrangian-remarks:fig:second-order-error}
\end{figure}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/stochastic-volatility/stochastic-volatility.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/stochastic-volatility/esjd.png}
  \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/stochastic-volatility/min-ess-per-second.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/stochastic-volatility/mean-ess-per-second.png}
  \caption{Mean ESS / Sec.}
  \end{subfigure}
  \caption{{\bf (Stochastic Volatility Model)} We show the ESJD and the minimum and mean ESS per second for the stochastic volatility model using HMC, RMHMC, LMC, and ILMC. In this example, ILMC moves less efficiently through the same space as measured by ESJD, and ultimately produces fewer effective samples per second relative to LMC. However, it is intriguing to note that ILMC nonetheless produces more effective transitions than RMHMC and HMC.}
  \label{lagrangian-remarks:fig:stochastic-volatility}
\end{figure*}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/t/t-5.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/t/esjd-dof-5.png}
  \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/t/ess-per-second-dof-5.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/t/ks-dof-5.png}
  \caption{Kolmogorov-Smirnov}
  \end{subfigure}
  \caption{{\bf (Multi-Scale Student-$t$ $\nu = 5\times 10^0$)} We show the ESJD, the minimum ESS per second, and the distribution of Kolmogorov-Smirnov statistics for sampling from the multiscale Student-$t$ distribution with $\nu=5\times 10^0$ using RMHMC, LMC, and ILMC. We observe that RMHMC enjoys the best ESJD, time-normalized ESS, and Kolmogorov-Smirnov statistics. This illustates an important limitation of the Lagrangian procedure in that its performance may actually be unable to match RMHMC in certain circumstances.}
  \label{lagrangian-remarks:fig:t-5}
\end{figure*}


==> Several Remarks on the Numerical Integrator in Lagrangian Monte Carlo(2)/figures/t/t-5000.tex <==
\begin{figure*}[t!]
  \centering
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/t/esjd-dof-5000.png}
  \caption{ESJD}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/t/ess-per-second-dof-5000.png}
  \caption{Min. ESS / Sec.}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.3\textwidth}
  \includegraphics[width=\textwidth]{images/t/ks-dof-5000.png}
  \caption{Kolmogorov-Smirnov}
  \end{subfigure}
  \caption{{\bf (Multi-Scale Student-$t$ $\nu = 5\times 10^3$)} We show the ESJD, the minimum ESS per second, and the distribution of Kolmogorov-Smirnov statistics for sampling from the multiscale Student-$t$ distribution with $\nu=5\times 10^3$ using RMHMC, LMC, and ILMC. In this example, despite having a smaller ESJD, ILMC ultimately produces a slight benefit in terms of ESS per second. Among the geometric methods, the distribution of the Kolmogorov-Smirnov statistics are nearly identical.}
  \label{lagrangian-remarks:fig:t-5000}
\end{figure*}

